Improving Dialog Systems for Negotiation with Personality Modeling

In this paper, we explore the ability to model and infer personality types of opponents, predict their responses, and use this information to adapt a dialog agent's high-level strategy in negotiation tasks. Inspired by the idea of incorporating a theory of mind (ToM) into machines, we introduce a probabilistic formulation to encapsulate the opponent's personality type during both learning and inference. We test our approach on the CraigslistBargain dataset and show that our method using ToM inference achieves a 20% higher dialog agreement rate compared to baselines on a mixed population of opponents. We also find that our model displays diverse negotiation behavior with different types of opponents.

==> method_original.tex <==
\section{Method}
\label{sec:model}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/tom_model}
    \caption{\runzhe{just a placeholder for now. we need to redraw a figure similar to this. basically it should contain sample utterance and dialogue act, with an emphasis of ToM inference.}}
    \label{fig:my_label}
\end{figure*}


\subsection{Modeling Negotiation as a Multi-Agent Markov Decision Process}
\label{sec:model:mdp}

We formulate the negotiation between two agents as the following multi-agent {\em Markov Decision Process} (MDP), $\langle \mathcal N, \mathcal S, \mathcal A, \mathcal P, \mathcal R, \Pi, n \rangle$:

$\mathcal N = \{-1, 1\}$ is the set indicating the identity of two agents. 
$\mathcal A$ is the action space consisting of different {\em dialogue acts}. 
Each dialogue act $a^i_t \in \mathcal A$ encodes the {\em intent} and {\em price} that the agent $i$ tries to express in the $t$-th round. 
Different from other simultaneous settings, two agents act alternatively, i.e., if the at round $t$ only the agent $i$ moves, then at round $t+1$ only the agent $-i$ move.

$\mathcal S$ is the state space consisting of the negotiation status. 
We define
$s_0 \in \mathcal S$ as the initial status of the dialogue, which contains the information about items to be negotiated (e.g., initial price, description). 
Also define $s_t = (s_0, a_{1}^{i}, a_{2}^{-i},  \dots,  a_{t-1}^{i}, a_{t}^{-i})$ to be the state at the end of round $t$. 
Note that the state $s_t$ is only partially observable in reality, since one can only infer the intent from the utterance. 
In our setting, we simplify the situation by assuming we have a perfect parser, which can translate the utterance to dialogue act $a_t$. 
Improving a parser or a language understanding module can be treated as an orthogonal research direction.

$\mathcal P$ is the transition probability from one state to another. In the negotiation setting, this is associated with agent policies $\Pi = \{\pi^{-i}, \pi^{i}\}$, where $\pi^{i}(a^{i}_{t}|s_{t-1}) = \pi^{i}(a^{i}_{t}|s_{t-1}, p^i)$ specify the probability of the agent $i$ choosing dialogue act $a^i_{t}$ at round $t$ based on previous dialogue statue and privacy $p^i$, e.g., the target price. Due to the special structure of the negotiation setting, we simplify notation to only use public state as the state of MDP, and hide the private state in the policy $pi$.
Since $s_{t}$ is the concatenation of $a^i_{t}$ and $s_{t-1}$, for simplicity we reuse the notation and define policy as $\pi^{i}(s_{t}|s_{t-1})$.

$\mathcal R = \{r^{-i}, r^{i}\}$ are the reward functions for two agents. $r^{i}(s_t, a^i_{t}) = r^{i}(s_{t+1})$ is zero until two parties reaches agreement to accept or reject an offer, or one party quite the negotiation. 
The negotiation start from round $t=1$ until the end or $t=n$, where $n$ is the length limit of dialogues. The goal of each agent is to find a policy which maximizes its own cumulative reward $\sum_{t=1}^{n}r^{i}_t(s_t,a^i_t)$, which can be approximately solved by reinforcement learning.

\subsection{A Modular Framework of Negotiation Systems}
Our framework is an extension of existing modular framework with coarse dialogue acts \cite{he2018emnlp}, which consists of three components: (1) A {\bf parse} translate the opponent's utterance $u^{-i}_{t-1}$ to dialogue act $a^{-i}_{t-1}$; (2) A {\bf dialogue manager} makes response $a^i_{t}$ based on state $s_{t-1} = (s_0, \dots, a^{-i}_{t-1})$. (3) A {\bf generator} produce an utterance $u^{i}_t$ conditioned on the $s_{t-1}$ and $a_t$ or equivalently $s_{t}$. 

The parser and the generator modules can be obtained by rule-based method or supervised learning in advance and fixed when training the dialogue manager using supervised learning (SL) or fine turning using reinforcement learning (RL). 

However, there are two may problems with previous dialogue policy. 
First, the policy learned by an RL-based dialogue manager produces reactive responses, which are usually lacking accuracy in a long term planning problem requiring more strategic thinking, such as negotiation. 
Second, it does not take the effect of our utterance into account.
To address these problems, we propose an incorporate the theory of mind (ToM) into the inference process to enabling one-step looking ahead to consider the effect of our utterances and generate more thoughtful strategies and also enables further fine-tuning the RL-based dialogue manager.

\subsection{Inference with First-Order Expected Theory of Mind (ToM)}
\label{sec:model:inference}
We introduce first-order expected ToM policy, $\pi_{\tt e}$, to the inference process. At the $t$-th round, key formula is as follows
\begin{equation*}
    \resizebox{0.50\textwidth}{!}{$\displaystyle
    \pi_{\tt e}(s_t | s_{t-1}) \propto \exp\left\{\frac{1}{\beta}\sum_{u_t}\underbrace{G(u_t|s_t)}_{\text{Generator}}\sum_{s_{t+1}} \underbrace{ T(s_{t+1}|s_t,u_t)}_{1^{\text{st}}\text{-order ToM}}\underbrace{V(s_{t+1})}_{\text{Value Fn.}}\right\},
    $}
\end{equation*}
where \runzhe{need one illustration here}
\begin{itemize}
    \item $T(s_{t+1}|s_t, u_t)$ is the {\bf first order ToM transition probability} from current $s_{t}$ and $u_t$ to the next state $s_{t+1}$, which can be estimated by supervised learning from the corpus. 
    \item $G(u_t|s_t)$ is the {\bf generator} which renders utterance conditioned on the current state (initial information and history of dialogue acts). It can be either deterministic to reduce computational cost or probabilistic to encourage diversity in language.
    \item $V(s_{t+1})$ is the {\bf value function} estimated by the RL-based dialogue manager, which gives the best future return estimation supposing the current state is $s_{t+1}$. To obtain this value, we need to use value based reinforcement learning method or actor-critic method.
    \item $\beta$ is the temperature parameter. Since $\pi_{\tt e}$ is normalized as a Boltzmann distribution, when temperature $\beta \rightarrow \infty$, $\pi_{\tt e}$ is uniform distribution, when  $\beta \rightarrow 0$, $\pi_{\tt e}$ is nearly deterministic assigning most probability mass to the $s_t$ with the largest expected ToM value.
\end{itemize}

This $\pi_{\tt e}$ is called first-order expected ToM policy, because it utilizes the first-order transition of the opponent, and estimate the expected outcome of performing a certain action leads to state $s_t$. In practice, the summation (expectation) is approximated by sampling.

And the final ToM policy in the 1st-order expected ToM inference is given by
\begin{equation*}
    \resizebox{0.38\textwidth}{!}{$\displaystyle
    \pi_{\tt ToM}(s_t|s_{t-1}) \propto \pi_{\tt rl}(s_t|s_{t-1}) \cdot \pi_{\tt e}(s_{t} | s_{t-1}),
    $}
\end{equation*}
where $\pi_{\tt rl}$ is the policy obtained by reinforcement learning in the previous training process. From a Bayesian point of view, $\pi_{\tt rl}$ can be seen as a prior $\mathbb P(s_t)$, and the $\pi_{\tt e}$ is analog to the likelihood $\mathbb P(\text{best return}|s_t)$ which modifies the probability assignment in $\pi_{\tt ToM}$, i.e., the posterior $\mathbb P(s_t|\text{best return})$. It reads that to reach the highest return in the end, what the probability that the current agent should move to $s_{t}$ is.

When $\beta \rightarrow 0$ in $\pi_{\tt e}$, we have a strong likelihood and the ToM policy is equivalent to find the best response that maximizes the expected total return after a 1-step move,
\begin{equation*}
    \resizebox{0.38\textwidth}{!}{$\displaystyle
    s_t^* = \argmax_{\substack{s_t=s_{t-1}\wedge a^i_t \\ a^i_t\in \mathcal A }}\expe_{\substack{u_t\sim G(\cdot|s_t)\\s_{t+1}\sim T(\cdot|u_t,s_t)}} \left[V(s_{t+1})\right].
    $}
\end{equation*}

Note that this is equivalent to maximizing  $\mathbb E[r(s_{t+1})+V(s_{t+1})]$ for any non-terminal state $s_{t+1}$ since in the our setting $r$ is always zero until the final state.

When $\beta \rightarrow \infty$, the likelihood is weak and in extreme we have $\pi_{\tt ToM} = \pi_{\tt rl}$. 

This ToM inference policy differs from the existing opponent modeling or model-based reinforcement learning method in two aspects: First, this can gain benefits from inference solely other than training, while opponent modeling and model-based RL methods are mainly gaining improvements from training process. Second, this method has the flexibility to adjust the degree that the final policy relies on the first-order ToM transition, which is robust even when the first-order ToM transition is noisy.

\subsection{Fine Tuning with First-Order Expected Theory of Mind (ToM)}
\label{sec:model:finetune}

We can also fine tune both $\pi_{\tt rl}$ and $\pi_{\tt e}$ using actor critic method. The actor tries to update the parameter of $\pi_{\tt rl}$ to maximize the expected total return. To update the parameter of $V$, i.e., $\theta_{k+1} \leftarrow \theta_k - \nabla_{\theta}\mathcal L(\theta)$, we use a critic loss function $\mathcal L(\theta)$ minimizing the temporal difference, which is 
\begin{equation*}
    \resizebox{0.48\textwidth}{!}{$\displaystyle
    \mathcal L(\theta) = \expe_{\tau \sim (\pi^i_{\tt ToM}, \pi^{-i})}\left[\expe_{\substack{u'_t\sim G(\cdot|s_t)\\s'_{t+1}\sim T(\cdot|u'_t,s_t)}}\left(\hat{r}(s_{t+1})+V_{\theta_k}(s'_{t+1})\right)-V_{\theta}(s_{t})\right]^2,
    $}
\end{equation*}
where the trajectory $\tau = (s_1, s_2, \dots, s_n)$ is sample from our ToM policy and the opponent's policy $(\pi^i_{\tt ToM}, \pi^{-i})$, and $\hat{r}$ is an empirical reward based on price difference. In practice, The outer expectation is sampled by interacting with another agent, and the inter expectation is simulated with our generator and ToM transition model. The inner simulation with ToM reduces the variance of one-step look ahead value estimation and leads to more efficient fine tuning.

The fine-tuning process can be seen as incorporating the ToM knowledge and linguistic property of the generator into training and the reactive policy $\pi_{\tt rl}$. When the system is interacting with a human, fine-tuning is necessary for adaptation.

\subsection{Game Theoretic Variants}
\label{sec:model:gametheory}

Inspired by game theory, the first-order expected ToM policy can two variants, {\bf competitive} ToM policy:
\begin{equation*}
    \resizebox{0.50\textwidth}{!}{$\displaystyle
    \pi_{\tt min}(s_t | s_{t-1}) \propto \exp\left\{\frac{1}{\beta}\sum_{u_t}\underbrace{G(u_t|s_t)}_{\text{Generator}}\min_{s_{t+1}} \underbrace{ T(s_{t+1}|s_t,u_t)}_{1^{\text{st}}\text{-order ToM}}\underbrace{V(s_{t+1})}_{\text{Value Fn.}}\right\},
    $}
\end{equation*}
and a {\bf cooperative} ToM policy:
\begin{equation*}
    \resizebox{0.50\textwidth}{!}{$\displaystyle
    \pi_{\tt max}(s_t | s_{t-1}) \propto \exp\left\{\frac{1}{\beta}\sum_{u_t}\underbrace{G(u_t|s_t)}_{\text{Generator}}\max_{s_{t+1}} \underbrace{ T(s_{t+1}|s_t,u_t)}_{1^{\text{st}}\text{-order ToM}}\underbrace{V(s_{t+1})}_{\text{Value Fn.}}\right\}.
    $}
\end{equation*}

The competitive ToM considers the worst case where the opponents take an unusual move to minimize our return, and the cooperative ToM considers the best case the other agent is always willing to improve our returns. 
Both situations can happen in real-life settings.
Tree search based algorithms are more like a competitive variant.

However, we argue that expected ToM is more suitable in the negotiation setting since both competitive and cooperative cases are too extreme. One party in the negotiation tends to be neutral -- to maximize its own utility (competitive) as well as find a price interval of agreement (cooperative).
